Narrowing your FOV with SOLiD: Spatially Organized and Lightweight Global Descriptor for FOV-constrained LiDAR Place Recognition

We often encounter limited FOV situations due to various factors such as sensor fusion or sensor mount in real-world robot navigation. However, the limited FOV interrupts the generation of descriptions and impacts place recognition adversely. Therefore, we suffer from correcting accumulated drift errors in a consistent map using LiDAR-based place recognition with limited FOV. Thus, in this paper, we propose a robust LiDAR-based place recognition method for handling narrow FOV scenarios. The proposed method establishes spatial organization based on the range-elevation bin and azimuth-elevation bin to represent places. In addition, we achieve a robust place description through reweighting based on vertical direction information. Based on these representations, our method enables addressing rotational changes and determining the initial heading. Additionally, we designed a lightweight and fast approach for the robot's onboard autonomy. For rigorous validation, the proposed method was tested across various LiDAR place recognition scenarios (i.e., single-session, multi-session, and multi-robot scenarios). To the best of our knowledge, we report the first method to cope with the restricted FOV. Our place description and SLAM codes will be released. Also, the supplementary materials of our descriptor are available at \texttt{\url{https://sites.google.com/view/lidar-solid}}.

==> PaperWriting/experiments.tex <==
\section{Results}
\subsection{Experiments Setup}
We present Histogram \cite{rohling2015fast}, M2DP \cite{he2016m2dp}, SC \cite{kim2018scan}, LoGG3D \cite{vidanapathirana2022logg3d}, OT \cite{ma2022overlaptransformer}, and Ring++ \cite{xu2023ring++} as comparative methods, generated using Python-based code to meet the same conditions.
% and all experiments are conducted on desktop Intel i7-12700 KF with RTX 3070Ti and onboard computer Jetson AGX Orin.
In our LiDAR \ac{PR} results, we employ a pre-trained model for learning-based OT and LoGG3D.
Our approach involves constructing a kd-tree, resulting in an approximately 8x faster searching time than brute-force searching based on the KITTI 00 dataset. 
However, for a fair comparison with all the methods except SC (owing to its hierarchical nature) in our experiments, we adopt a brute-force search, not efficient search techniques (e.g. radius search, kd-tree).
Furthermore, to assess the effects of vertical resolution and scan pattern based on LiDAR type, we conduct experiments using various datasets including different channels (e.g. 16 or 64) and solid-state LiDAR.
In addition, we define the processing time as the average descriptor generation time (raw scan $\rightarrow$ descriptor) $+$ the average loop searching time (current descriptor $\&$ database $\rightarrow$ candidate index).
In each performance evaluation, we designate the \bl{\textbf{first rank}} in bold blue and the \textbf{second rank} in bold.

\subsection{Comparison of Description}
\begin{table}[h]
\caption{Comparison of LiDAR Place Recognition for Loop Detection}
\renewcommand{\arraystretch}{1.5}
\centering\resizebox{0.48\textwidth}{!}{
{\huge
\begin{tabular}{l|ccccccc}
\toprule \hline
Descriptor       & Hist. (C)          & LoGG3D (G) & M2DP (C)     & SC (C)             & OT (G)      & Ring++ (G)   & Ours (C) \\ \hline
Size [bytes]     & \textbf{928}       & 2176       & 1664         & 10016              & 1152        & 345728       & \bl{\textbf{448}}  \\
CPU Only        & \checkmark         & {x}        & \checkmark   & \checkmark         & {x}         & {x}          & \checkmark    \\
Initial Guess    & {x}                &  {x}       & {x}          & \checkmark         & {x}         & \checkmark   & \checkmark    \\ \hline \bottomrule
\end{tabular}}}
\label{table:description}
% \vspace{-1cm}
\end{table}

As listed in \tabref{table:description}, we compare the descriptor size and requirements of the GPU to investigate whether it is lightweight and efficient. 
In addition, we check the possibility of initial pose estimation to enhance the \ac{ICP} performance.
First, we denote the methods that can be performed with only a CPU as (C) and those that require a GPU as (G).
Similar to other handcrafted methodologies, our method does not require a GPU but possesses an extremely lightweight descriptor.
In contrast to other 1D methodologies (Histogram, LoGG3D, M2DP, and OT), the proposed approach can estimate the initial guess.

\begin{table*}[t]
\caption{Evaluation for single-session LiDAR Place Recognition}
% \renewcommand{\arraystretch}{1.2}
\centering\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc}
\toprule \hline
\multicolumn{14}{c}{Sequence}                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{FOV}}      & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{4}{c|}{00 (4541 frames)}  & \multicolumn{4}{c|}{02 (4661 frames)} & \multicolumn{4}{c}{05 (2761 frames)}\\ \cline{3-14} 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{}           & Recall@1                                & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1 max} & \multicolumn{1}{c|}{Time [Hz]}              
                                                                                 & \multicolumn{1}{c}{Recall@1}            & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1 max} & \multicolumn{1}{l|}{Time [Hz]} 
                                                                                 & \multicolumn{1}{c}{Recall@1}            & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1 max} & Time [Hz] \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{60}}       & \multicolumn{1}{c|}{Hist. (C)}  & \multicolumn{1}{c}{0.764}               &0.965                    &0.754                       & \multicolumn{1}{c|}{3.06}          
                                                                                 & 0.483                                   &0.960                    &0.452                       & \multicolumn{1}{c|}{3.05}     
                                                                                 & 0.611                                   &0.949                    &0.606                       & 3.21     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Logg3D (G)} & \multicolumn{1}{c}{0.726}               &0.914                    &0.552                       & \multicolumn{1}{c|}{30.76}
                                                                                 & 0.674                                   &0.954                    &0.627                       & \multicolumn{1}{c|}{30.59}
                                                                                 & 0.593                                   &0.936                    &0.531                       & 33.55     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{M2DP (C)}   & \multicolumn{1}{c}{0.703}               &0.935                    &0.664                       & \multicolumn{1}{c|}{15.40}
                                                                                 & 0.471                                   &0.972                    &0.469                       & \multicolumn{1}{c|}{15.36}
                                                                                 & 0.468                                   &0.969                    &0.517                       & 15.96     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{SC (C)}     & \multicolumn{1}{c}{0.547}               &0.577                    &0.220                       & \multicolumn{1}{c|}{3.24}
                                                                                 & 0.177                                   &0.116                    &0.031                       & \multicolumn{1}{c|}{3.24}
                                                                                 & 0.373                                   &0.399                    &0.159                       & 3.29     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{OT (G)}     & \multicolumn{1}{c}{0.740}               &0.964                    &0.708                       & \multicolumn{1}{c|}{\textbf{\bl{135.14}}}
                                                                                 & 0.651                                   &0.946                    &0.574                       & \multicolumn{1}{c|}{\textbf{\bl{133.51}}}
                                                                                 & 0.540                                   &0.958                    &0.553                       & \textbf{\bl{164.74}}     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ring++ (G)} & \multicolumn{1}{c}{\textbf{\bl{0.834}}} &\textbf{0.982}           &\textbf{\bl{0.831}}         & \multicolumn{1}{c|}{0.45}
                                                                                 & \textbf{0.701}                          &\textbf{\bl{0.993}}      &\textbf{0.729}              & \multicolumn{1}{c|}{0.44}
                                                                                 & \textbf{\bl{0.688}}                     &\textbf{0.974}           &\textbf{\bl{0.753}}         & 0.76    \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ours (C)}   & \multicolumn{1}{c}{\textbf{0.800}}      &\textbf{\bl{0.987}}      &\textbf{0.830}              & \multicolumn{1}{c|}{\textbf{57.94}}
                                                                                 & \textbf{\bl{0.706}}                     &\textbf{0.990}           &\textbf{\bl{0.746}}         & \multicolumn{1}{c|}{\textbf{57.34}}
                                                                                 & \textbf{0.639}                          &\textbf{\bl{0.992}}      &\textbf{0.732}              & \textbf{68.40}    \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{120}}      & \multicolumn{1}{c|}{Hist. (C)}  & \multicolumn{1}{c}{0.780}               &0.961                    &0.771                       & \multicolumn{1}{c|}{1.57}
                                                                                 & 0.483                                   &0.965                    &0.427                       & \multicolumn{1}{c|}{1.57}
                                                                                 & 0.596                                   &0.958                    &0.613                       & 1.61     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Logg3D (G)} & 0.746                                   &0.920                    &0.581                       & \multicolumn{1}{c|}{26.15} 
                                                                                 & 0.674                                   &0.983                    &0.664                       & \multicolumn{1}{c|}{26.03} 
                                                                                 & 0.625                                   &0.910                    &0.511                       & 28.14     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{M2DP (C)}   & 0.751                                   &0.959                    &0.728                       & \multicolumn{1}{c|}{8.67}
                                                                                 & 0.404                                   &\textbf{0.987}           &0.441                       & \multicolumn{1}{c|}{8.66}
                                                                                 & 0.460                                   &\textbf{0.978}           &0.525                       & 8.85     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{SC (C)}     & 0.417                                   &0.393                    &0.152                       & \multicolumn{1}{c|}{3.21}
                                                                                 & 0.151                                   &0.155                    &0.045                       & \multicolumn{1}{c|}{3.20}
                                                                                 & 0.332                                   &0.379                    &0.126                       & 3.25     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{OT (G)}     & 0.799                                   &0.927                    &0.705                       & \multicolumn{1}{c|}{\textbf{\bl{97.18}}}
                                                                                 & 0.691                                   &0.969                    &0.616                       & \multicolumn{1}{c|}{\textbf{\bl{96.33}}}
                                                                                 & 0.614                                   &0.891                    &0.516                       & \textbf{\bl{111.61}}     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ring++ (G)} & \textbf{\bl{0.862}}                     &\textbf{0.977}           &\textbf{\bl{0.880}}         & \multicolumn{1}{c|}{0.45}
                                                                                 & \textbf{\bl{0.750}}                     &0.978                    &\textbf{\bl{0.815}}         & \multicolumn{1}{c|}{0.44}
                                                                                 & \textbf{\bl{0.732}}                     &0.974                    &\textbf{\bl{0.793}}         & 0.75     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ours (C)}   & \textbf{0.822}                          &\textbf{\bl{0.994}}      &\textbf{0.868}              & \multicolumn{1}{c|}{\textbf{45.19}}
                                                                                 & \textbf{0.735}                          &\textbf{\bl{0.992}}      &\textbf{0.790}              & \multicolumn{1}{c|}{\textbf{44.82}}
                                                                                 & \textbf{0.656}                          &\textbf{\bl{0.989}}      &\textbf{0.737}              & \textbf{51.31}     \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{180}}       & \multicolumn{1}{c|}{Hist. (C)} & \multicolumn{1}{c}{0.780}               &0.966                    &0.761                       & \multicolumn{1}{c|}{1.09}
                                                                                 & 0.462                                   &0.965                    &0.410                       & \multicolumn{1}{c|}{1.08}
                                                                                 & 0.542                                   &0.952                    &0.570                       & 1.10     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Logg3D (G)} & 0.780                                   &0.918                    &0.609                       & \multicolumn{1}{c|}{22.87}
                                                                                 & 0.701                                   &0.966                    &0.647                       & \multicolumn{1}{c|}{22.77}
                                                                                 & 0.611                                   &0.903                    &0.492                       & 24.37     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{M2DP (C)}   & 0.739                                   &0.940                    &0.694                       & \multicolumn{1}{c|}{6.03}
                                                                                 & 0.523                                   &0.981                    &0.555                       & \multicolumn{1}{c|}{6.02}
                                                                                 & 0.497                                   &0.921                    &0.526                       & 6.11     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{SC (C)}     & 0.547                                   &0.577                    &0.694                       & \multicolumn{1}{c|}{3.16}
                                                                                 & 0.177                                   &0.116                    &0.031                       & \multicolumn{1}{c|}{3.16}
                                                                                 & 0.384                                   &0.353                    &0.146                       & 3.21     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{OT (G)}     & \textbf{0.842}                          &0.907                    &0.719                       & \multicolumn{1}{c|}{\textbf{\bl{76.34}}}
                                                                                 & 0.698                                   &0.962                    &0.646                       & \multicolumn{1}{c|}{\textbf{\bl{75.82}}}
                                                                                 & 0.645                                   &0.864                    &0.466                       & \textbf{\bl{84.96}}     \\
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ring++ (G)} & \textbf{\bl{0.895}}                     &\textbf{0.976}           &\textbf{\bl{0.887}}         & \multicolumn{1}{c|}{0.45}
                                                                                 & \textbf{\bl{0.752}}                     &\textbf{0.983}           &\textbf{\bl{0.813}}         & \multicolumn{1}{c|}{0.44}
                                                                                 & \textbf{\bl{0.744}}                     &\textbf{\bl{0.988}}      &\textbf{\bl{0.795}}         & 0.74     \\ 
\multicolumn{1}{c|}{}                          & \multicolumn{1}{c|}{Ours (C)}   & 0.840                                   &\textbf{\bl{0.994}}      &\textbf{0.868}              & \multicolumn{1}{c|}{\textbf{37.61}}
                                                                                 & \textbf{0.735}                          &\textbf{\bl{0.990}}      &\textbf{0.799}              & \multicolumn{1}{c|}{\textbf{37.36}}
                                                                                 & \textbf{0.659}                          &\textbf{0.974}           &\textbf{0.710}              & \textbf{41.75}  \\ \hline \bottomrule
\end{tabular}}
\vspace{-0.1cm}
\label{table:eval_pr}
\end{table*}

% We utilize the KITTI \cite{geiger2012we}, HeLiPR \cite{jung2023helipr}, and PARK \cite{huang2021disco} datasets to demonstrate the robustness of our approach not only in single-sessions but also in multi-session and distributed session scenarios for PR. 
% To make the KITTI and PARK datasets equipped with spinning \ac{LiDAR} comparable to solid-state \ac{LiDAR}, we conduct experiments by clipping the data to include perspectives at various FOVs (60$^\circ$, 120$^\circ$, 180$^\circ$, and occlusion) as shown in \figref{fig:various_fov}.

% In designing loop detection, we configure it to search in all previously revisited places except for the most recent 100 frames.

% \begin{itemize}
%     \item \textit{KITTI} datasets include driving sequences involving cars with Velodyne HDL-64E \ac{LiDAR} and serve as the foundation for various PR evaluations. 
%                   In our evaluation, we utilize sequences \textit{00}, \textit{02}, \textit{05} for overall performance and \textit{08} for pose estimation evaluation.
%     \item \textit{HeLiPR} datasets are acquired using various types of \ac{LiDAR} setups installed on cars. Specifically, we focus on the solid-state Aeva Aeries                                            \uppercase\expandafter{\romannumeral2} and Livox Avia \ac{LiDAR}s, utilizing sequences from \textit{Town1}, \textit{Town2}, \textit{RoundAbout1}, \textit{RoundAbout2},                     \textit{KAIST04}, and \textit{KAIST05}.
%                   Among these, \textit{Town2}, \textit{RoundAbout2}, and \textit{KAIST05} are selected as targets that have the increased complexity caused by dynamic objects. 
%                   Additionally, we conduct inter-session experiments, sampling poses at 2 meters.
%     \item \textit{PARK} datasets serve as a performance metric for DISCO SLAM \cite{huang2021disco} and involve the operation of three robots, each equipped with Velodyne VLP-16 \ac{LiDAR}.                 We conduct pose sampling at 2 meters and utilize these datasets to showcase results in a distributed session. 
%                   In particular, in this dataset, individuals acquiring data with mobile robots exist as dynamic objects.
% \end{itemize}

\subsection{Single-Session LiDAR Place Recognition Evaluation}
We utilize well-known \textit{KITTI} \cite{geiger2012we} datasets to evaluate the single-session LiDAR \ac{PR} performance.
\textit{KITTI} datasets include driving sequences involving cars with Velodyne HDL-64E LiDAR and serve as the foundation for various LiDAR \ac{PR} evaluations. 
In our evaluation, we utilize sequences \textit{00}, \textit{02}, \textit{05} for the overall performance of limited FOV with occlusions as shown in  \figref{fig:various_fov}.
We compare the runtime on a desktop Intel i7-12700 KF with RTX 3070Ti and an onboard computer Jetson AGX Orin at limited FOV.
Also, the \textit{08} sequence is utilized for pose estimation evaluation.
We set the criteria for determining the true positive (TP) loops and false positive (FP) loops to within 10m, and the most recent 100 frames are excluded from the candidate pool.
% (i.e. average descriptor generation time + average loop searching time)
\begin{figure}[h]
    \centering
    \def\width{0.98\columnwidth}
    \includegraphics[clip, trim= 20 220 20 180, width=\width]{Figure/various_fov/various_fov.pdf}
    \caption{500th frame from various angles in \textit{KITTI 00}. Black represents full view (360$^\circ$) points. Blue, green, yellow, and red mean occlusion, 180$^\circ$, 120$^\circ$, and 60$^\circ$ points, respectively.}
    % \vspace{-0.8cm}
    \label{fig:various_fov}
\end{figure} 

%% ROC curve
%% ===========================================================================================================================================================================
\begin{figure}[t]
    \centering
    \def\width{1\columnwidth}
    \includegraphics[clip, trim= 60 640 60 10, width=\width]{Figure/roc_curve/roc_curve.pdf}
    \caption{The ROC curves when LiDAR is occluded. Left is \textit{KITTI 00}, and right is \textit{KITTI 02}.}
    \vspace{-0.5cm}
    \label{fig:roc_curve}
\end{figure} 
%% ===========================================================================================================================================================================

\subsubsection{Overall performance}
As shown in \tabref{table:eval_pr}, we utilize metrics, such as the Recall@1, AUC score, F1 max score, and processing time to evaluate the LiDAR \ac{PR}.
% To facilitate usage in various tasks within a limited FOV, experiments are conducted on a modified \textit{KITTI} dataset by applying clipping as shown in \figref{fig:various_fov}.
% Based on these discussions
The overall metrics show a competitive comparison between Ring++ and our SOLiD, demonstrating comparable performance.
Considering the Recall@1 and F1 max score, Ring++ generally outperformed, indicating that it tends to discover more loops than our method.
However, from the perspective of LiDAR \ac{PR} improving SLAM errors to enhance map accuracy, it is crucial to prioritize more accurate loops over a higher number of loops. 
This is reflected in the AUC score, where our approach demonstrated a noticeable improvement. 
In addition, while Ring++ is unsuitable for real-time applications as it averages approximately 0.5 Hz, our method, which averages approximately 50 Hz, is more effective for real-time deployment in large-scale robotic systems because its performance is 100$\times$ faster than that of Ring++.
In particular, it can be observed that histograms or M2DP, which involve more compression, experience an exponential increase in time. 
Moreover, the search time is inherently long for the SC (2D) and Ring++ (3D) matrix approaches.
In contrast, our method demonstrates real-time performance, and Sections \uppercase\expandafter{\romannumeral4}-~C consistently confirm its high performance even with clipping.
% A noteworthy point is that the descriptors become faster to apply on robot platforms as points get more clipped. 
% When comparing the metrics at or near real-time performance for each method, our approach stands out with overwhelmingly superior performance.
%% ===========================================================================================================================================================================

%% Matching Graph
%% ===========================================================================================================================================================================
\begin{figure*}[t]
    \centering
    \def\width{2\columnwidth}
    \includegraphics[clip, trim= 0 250 0 60, width=\width]{Figure/matching_graph/matching_graph.pdf}
    \caption{3D matching pair graph when each descriptor's precision is highest in PR-curve of \textit{HeLiPR} dataset (target: \textit{KAIST04}, source: \textit{KAIST05}). Green represents true matching pairs, and red represents false matching pairs.}
    \vspace{-0.3cm}
    \label{fig:matching_Graph}
\end{figure*}
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsubsection{Robustness of Occlusion}
Occlusions caused by a LiDAR malfunction have a significant adverse impact on robot navigation.
Occlusion of LiDAR leads to information loss, directly contributing to errors in LiDAR odometry.
Therefore, although extensive exploration is important, a LiDAR \ac{PR} that can accurately distinguish between revisited places is even more crucial.
We present the Receiver operating characteristic (ROC) curve in \figref{fig:roc_curve}, which is an appropriate metric for assessing performance.
\noindent ROC curve illustrates the relationship between \textit{sensitivity (SE)} and \textit{1-specificity (SP)}. 
Sensitivity represents the TP rate, and specificity denotes the FP rate.
The ROC curve is used to assess the performance of the model, with a larger AUC score, indicating superior ability.
As is evident from the ROC curve when occlusion occurs, our method shows superior performance compared to the other approaches.
This performance implies that, even with reduced information owing to occlusion at certain angles, the proposed method can still assist in minimizing odometry errors in \ac{SLAM}.
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsubsection{Initial Pose Estimation}
When the field of view (FOV) is limited, it is common to encounter cases where the difference in distance exceeds 10m when identifying reverse loops.
To reduce this ambiguity, we evaluate the performance of our initial rotation on the \textit{KITTI 08} dataset with a full view ($360^\circ$).
We analyze the RMSE when predicting the initial rotation of our method, employing the \ac{ICP} algorithm.
The RMSE is approximately \textbf{1.05}m when no initial values are provided. 
However, when initial values are provided, the RMSE decreases to around \bl{\textbf{0.50}}m, indicating a reduction of approximately two folds.
In essence, our \textit{A-SOLiD} can accurately estimate the initial pose with only a one-dimensional description, contributing to an improvement in the performance of the \ac{SLAM}.
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsubsection{Runtime}
% 실제 사용하는데 있어서 도움을 줄 수 있다는 내용 추가하기.
We compare the processing times for various limited FOVs using an onboard computer.
In practical applications, such as robot navigation, it is common to use a mobile platform and employ an onboard computer tailored to the size of the robot.
Therefore, it is expected that these metrics will be valuable for the robotics industry.
\tabref{table:fov_time} shows that the OT exhibits the fastest processing time. 
Although the Jetson AGX Orin allows performance measurement owing to its GPU presence, most onboard computers lack a GPU, prohibiting the use of OT.
Therefore, our methodology is not only independent of GPU constraints but is also particularly well-suited for use on onboard computers owing to its speed.
% \tabref{table:fov_time} illustrates a decrease in time on the onboard computer as the extent of clipping increases.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{Processing Time to LiDAR's FOV on Onboard Computer}
\renewcommand{\arraystretch}{1.2}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|ccccccc}
\toprule \hline
\multirow{2}{*}{Computer}      & \multirow{2}{*}{FOV} & \multicolumn{7}{c}{Processing Time {[}s{]}}                                     \\ \cline{3-9} 
                               &                      & Hist. (C) & LoGG3D (G) & M2DP (C) & SC (C) & OT (G)               & Ring++ (C) & Ours (C) \\ \hline
\multirow{4}{*}{Onboard Comp.} & 60                   & 1.289     & 0.160      & 0.297    & 1.359  & \bl{\textbf{0.036}}  & 10.85      & \textbf{0.073}    \\
                               & 120                  & 2.442     & 0.188      & 0.531    & 1.371  & \bl{\textbf{0.047}}  & 10.92      & \textbf{0.093}    \\
                               & 180                  & 3.550     & 0.215      & 0.710    & 1.382  & \bl{\textbf{0.056}}  & 10.98      & \textbf{0.111}    \\
                               & 360                  & 6.996     & 0.312      & 1.136    & 1.440  & \bl{\textbf{0.083}}  & 11.16      & \textbf{0.200}    \\ \hline \bottomrule
\end{tabular}}
\vspace{-0.5cm}
\label{table:fov_time}
\end{table}
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
% multi-session time evaluation
% We measure the processing time according to the \ac{LiDAR} type on both desktop and onboard computers as shown in \tabref{table:helipr_time} in \textit{HeLiPR Town1-Town2} sequences. 
% While our method mostly maintains the second position compared to OT and LoGG3D, those methods require a training process.
%% ===========================================================================================================================================================================
%% ===========================================================================================================================================================================
\subsection{Multi-Session LiDAR Place Recognition Evaluation}
We evaluate the performance of multi-session LiDAR \ac{PR} targeting Aeva and Avia using the \textit{HeLiPR} datasets.
\textit{HeLiPR} datasets are acquired using various types of LiDAR setups installed in cars.
Specifically, we focus on solid-state Aeva Aeries \uppercase\expandafter{\romannumeral2} and Livox Avia LiDAR, utilizing sequences from \textit{Town1}, \textit{Town2}, \textit{RoundAbout1}, \textit{RoundAbout2}, \textit{KAIST04}, and \textit{KAIST05}.
Among these, \textit{Town2}, \textit{RoundAbout2}, and \textit{KAIST05} are selected as targets with increased complexities caused by dynamic objects. 
In multi-session scenarios, frequent changes in a scene, such as change detection and incremental mapping, pose challenges.
Therefore, a precise LiDAR \ac{PR} is required.
We examine the 3D matching graph and the corresponding numbers when the precision is at its highest. 
In addition, we plot a PR (Precision-Recall)-curve to evaluate the consistent performance and monitor runtime on an onboard computer.
Additionally, we conduct multi-session experiments by sampling poses 2m apart.
A loop is considered a TP loop if it is detected within 5m.
In contrast to several other experiments that accumulated Avia's pointclouds \cite{jung2023helipr}, we conduct experiments using raw point clouds without pre-processing. 
This is because we believe that the accumulation of Avia's pointclouds is inefficient.

%% ===========================================================================================================================================================================
\subsubsection{Matching Graph \& Number}
% Multi-session scenarios prove to be valuable in map merging. 
% In map merging, a false matching pair can distort the map, therefore, the accuracy of true matching pairs is crucial. 
As depicted in \figref{fig:matching_Graph}, the proposed method shows that there are no false matching pairs.
Quantitatively, our approach exhibits a substantial number of true matching pairs without false matching pairs, as shown in \tabref{table:matching_number}.
In particular, Ring++ is vulnerable to dense horizontal information from the Aeva LiDAR.
Because Ring++ relies on geometric features such as eigenvalues, dynamic objects can introduce significant confusion into these features.
Although RT may be more robust with sparse information, chaos can be introduced in dense information scenarios.
\begin{table}[h]
\caption{Number of Matching Pair in KAIST04-KAIST05}
\renewcommand{\arraystretch}{1.2}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|ccccccc}
\toprule \hline
LiDAR Type            & Desc.             & Hist. (C)     & LoGG3D (G)  & M2DP (C)     & SC (C)         & OT (G)      & Ring++ (G)  & Ours (C) \\ \hline
\multirow{2}{*}{Aeva} & TP $\uparrow$     & 536           & 5           & 165          & 1099           & 12          & 63          & 1206    \\
                      & FP $\downarrow$   & 0             & 10          & 0            & 1195           & 1           & 0           & 0    \\ \hline
\multirow{2}{*}{Avia} & TP $\uparrow$     & 197           & 1           & 6            & 1099           & 108         & 536         & 400    \\
                      & FP $\downarrow$   & 0             & 2           & 0            & 326            & 33          & 0           & 0    \\ \hline \bottomrule
\end{tabular}}
\label{table:matching_number}
% \vspace{-0.5cm}
\end{table}
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsubsection{Precision-Recall Curve}
\figref{fig:pr_curve} shows the PR-Curve.
Learning-based techniques exhibit vulnerable performance owing to changes in LiDAR types.
In addition, it can be observed that 1D methods, such as Histogram and M2DP, which do not have empty spaces, demonstrate better performance than SC (2D), which has a significant presence of vacant spaces.

\begin{figure}[h]
    \centering
    \def\width{1\columnwidth}
    \includegraphics[clip, trim= 0 340 0 20, width=\width]{Figure/pr_curve/pr_curve.pdf}
    \caption{PR-Curve on \textit{HeLiPR} datasets. The left column uses Aeva LiDAR and the right uses Avia LiDAR.
             Moreover, the top represents \textit{KAIST04}-\textit{KAIS05}, the middle means \textit{Town1}-\textit{Town2} and the bottom means \textit{RoundAbout01}-\textit{RoundAbout02} session.}
    % \vspace{-0.5cm}
    \label{fig:pr_curve}
\end{figure} 

\subsubsection{Runtime}
The proposed method and Ring++ outperform the other methods, as shown in \figref{fig:pr_curve}.
When considering the real-time aspect relative to their performance, Ring++ falls short in time efficiency; however, our approach demonstrates real-time feasibility, as deduced in \tabref{table:helipr_time}.
Considering the trade-off between performance and processing time, our proposed approach proves to be suitable.
\begin{table}[h]
\caption{Processing Time according to LiDAR Type}
\renewcommand{\arraystretch}{1.2}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|ccccccc}
\toprule \hline
\multirow{2}{*}{Computer}        & \multirow{2}{*}{LiDAR Type} & \multicolumn{7}{c}{Processing Time {[}s{]}}         \\ \cline{3-9} 
                                 &                                                     & Hist. (C) & LoGG3D (G)               & M2DP (C)   & SC (C)     & OT (G)             & Ring++ (G) & Ours (C)                   \\ \hline
\multirow{2}{*}{Onboard Comp.}
                                 
                                 & Aeries \uppercase\expandafter{\romannumeral2}  & 5.291     & 0.229                & 1.109  & 1.439  & \bl{\textbf{0.083}}  & 15.70  & \textbf{0.143}    \\
                                 & Avia                                           & 1.260     & 0.189                & 0.258  & 1.433  & \bl{\textbf{0.047}}  & 15.58  & \textbf{0.137}   \\ \hline
\multirow{2}{*}{Desktop}         
                                 
                                 & Aeries \uppercase\expandafter{\romannumeral2}  & 1.426     & 0.056                & 0.271  & 0.145  & \bl{\textbf{0.021}}  & 3.720  & \textbf{0.036}    \\
                                 & Avia                                           & 0.323     & 0.039                & 0.072  & 0.142  & \bl{\textbf{0.012}}  & 3.680  & \textbf{0.033}    \\ \hline\bottomrule
\end{tabular}}
\label{table:helipr_time}
\vspace{-0.5cm}
\end{table}

%% ===========================================================================================================================================================================
% \subsubsection{Cope with Dynamic Object}
% Furthermore, we qualitatively verify the robustness of our method against noise and dynamic objects.
% In the scenario where a dynamic object exists within a single 3D bin, if $N_r$ is 40, and $N_e$ is 60.
% Consequently, each element of a value in SOLiD occupies a proportion of approximately 0.042$\%$ (1/2400). 
% This suggests that the influence of dynamics on the descriptor is considered to be minimal.
% % inter-session dyanmic
% \begin{figure}[h]
%     \centering
%     \def\width{0.98\columnwidth}
%     \includegraphics[clip, trim= 0 300 300 0, width=\width]{Figure/multi_session_dynamic/multi_session_dynamic.pdf}
%     \caption{A true loop scene with the presence of dynamic objects.}
%     \vspace{-0.2cm}
%     \label{fig:dynamic}
% \end{figure} 

% \noindent \figref{fig:dynamic} illustrates successful matching despite the presence of dynamic objects.
% Therefore, the successful operation of our ray weight indicates effective functionality.
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsection{Multi-Robot Session LiDAR Place Recognition Evaluation}
We conduct evaluations using the multi-robot session \textit{PARK} datasets.
\textit{PARK} datasets serve as a performance metric for the DISCO SLAM \cite{huang2021disco} and involve the operation of three robots, each equipped with a Velodyne VLP-16 LiDAR.   
We test the overall performance for various limited FOVs, similar to single-session evaluation.
In a multi-robot session, it is possible to obtain a map effectively using multiple robots.
However, for this to hold significance, smooth communication between the robots is essential. 
If such conditions are not satisfied, obtaining a map using multiple robots may not differ significantly from obtaining a map using a single robot.
Therefore, we measure the communication times for loop detection to evaluate the communication capabilities among the robots.
We conduct pose sampling at 2m and utilize these datasets to showcase the results in a multi-robot session. 
The TP loop is defined as 5m.
% In particular, in this dataset, individuals acquiring data with mobile robots exist as dynamic objects.

\subsubsection{Overall Performance}
\tabref{table:dist_eval} presents the experimental results in the multi-robot session, including the Recall@1, AUC score, F1 max score and communication time.
The experiment yields results for each robot paired with two distinct robots. 
Therefore, we obtain the results by averaging the outcomes of the six experiments, as shown in \tabref{table:dist_eval}.
Ring++ and the proposed approach outperform the other methods. 
In particular, despite the dataset being specialized for SC, it is evident that vacant areas are vulnerable.

\subsubsection{Communication Time}
When measuring the communication time, we assume that each robot is equipped with a Jetson AGX Orin, Intel NUC 10 Performance Mini PC, and Intel NUC 12 Pro Mini PC.
Our scenario assumes exchanging all acquired descriptors for loop matching, and we aggregate the results of 6 experiments to derive the final communication time.
We measure the bandwidth accordingly and also assume that there are no restrictions on the communication distance.
The heavyweight descriptor size of Ring++ results in a communication time of approximately 106s, whereas the lightweight descriptor size of our approach is approximately 0.138s, which is approximately 1000$\times$ faster than that of Ring++.

\begin{table}[h]
\caption{Evaluation for Multi-Robot Session LiDAR Place Recognition}
% \renewcommand{\arraystretch}{1.2}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|ccc|c}
\toprule \hline
Method                     & FOV                      & Recall@1$\uparrow$   & AUC$\uparrow$       & F1 max$\uparrow$     & Commu. Time $\downarrow$ \\ \hline
\multirow{3}{*}{Hist. (C)} & \multicolumn{1}{c|}{60}  & 0.405                & 0.847               & 0.349                & \multirow{3}{*}{\textbf{0.285}s}          \\
                           & \multicolumn{1}{c|}{120} & 0.431                & 0.862               & 0.373                &                            \\
                           & \multicolumn{1}{c|}{180} & 0.465                & 0.856               & 0.375                &                            \\ \hline
\multirow{3}{*}{LoGG3D (G)}& \multicolumn{1}{c|}{60}  & \textbf{0.590}       & 0.843               & 0.387                & \multirow{3}{*}{0.669s}          \\
                           & \multicolumn{1}{c|}{120} & 0.647                & 0.890               & 0.471                &                            \\
                           & \multicolumn{1}{c|}{180} & 0.654                & 0.910               & 0.516                &                            \\ \hline
\multirow{3}{*}{M2DP (C)}  & \multicolumn{1}{c|}{60}  & 0.379                & 0.874               & 0.359                & \multirow{3}{*}{0.511s}          \\
                           & \multicolumn{1}{c|}{120} & 0.433                & \textbf{0.919}      & 0.417                &                            \\
                           & \multicolumn{1}{c|}{180} & 0.432                & 0.888               & 0.383                &                            \\ \hline
\multirow{3}{*}{SC (C)}    & \multicolumn{1}{c|}{60}  & 0.474                & 0.648               & 0.272                & \multirow{3}{*}{3.077s}          \\
                           & \multicolumn{1}{c|}{120} & 0.468                & 0.579               & 0.272                &                            \\
                           & \multicolumn{1}{c|}{180} & 0.497                & 0.570               & 0.278                &                            \\ \hline
\multirow{3}{*}{OT (G)}    & \multicolumn{1}{c|}{60}  & 0.366                & 0.867               & 0.348                & \multirow{3}{*}{0.354s}          \\
                           & \multicolumn{1}{c|}{120} & 0.423                & 0.834               & 0.369                &                            \\
                           & \multicolumn{1}{c|}{180} & 0.482                & 0.864               & 0.395                &                            \\ \hline
\multirow{3}{*}{Ring++ (G)}& \multicolumn{1}{c|}{60}  & \textbf{\bl{0.670}}  & \textbf{\bl{0.940}} & \textbf{\bl{0.585}}  & \multirow{3}{*}{106.221s}          \\
                           & \multicolumn{1}{c|}{120} & \textbf{\bl{0.701}}  & \textbf{\bl{0.975}} & \textbf{\bl{0.730}}  &                            \\
                           & \multicolumn{1}{c|}{180} & \textbf{\bl{0.707}}  & \textbf{\bl{0.986}} & \textbf{\bl{0.767}}  &                             \\ \hline
\multirow{3}{*}{Ours (C)}  & \multicolumn{1}{c|}{60}  & 0.572                & \textbf{0.881}      & \textbf{0.442}       & \multirow{3}{*}{\textbf{\bl{0.138}}s}          \\
                           & \multicolumn{1}{c|}{120} & \textbf{0.665}       & \textbf{0.919}      & \textbf{0.548}       &                            \\
                           & \multicolumn{1}{c|}{180} & \textbf{0.689}       & \textbf{0.930}      & \textbf{0.571}       &                            \\ \hline \bottomrule
\end{tabular}}
\label{table:dist_eval}
\vspace{-0.2cm}
\end{table}
%% ===========================================================================================================================================================================

%% ===========================================================================================================================================================================
\subsection{Ablation Study}
The key components of the descriptor are $N_r$ and $N_e$.
These values determine the spatial definition, and we conduct an ablation study to investigate its impact.
\tabref{table:abs_rsolid} illustrates the LiDAR \ac{PR} performance of \textit{R-SOLiD} as it varies with $N_r$ and $N_e$ in \textit{KITTI 00}.
While there is some variation based on the values, it can be observed that the changes are negligible, indicating that heuristic efforts through parameter tuning are not crucial.
\begin{table}[h]
\caption{Ablation Study for R-SOLiD}
\renewcommand{\arraystretch}{1.2}
\centering\resizebox{0.48\textwidth}{!}{
\begin{tabular}{c|c|cccccc}
\toprule \hline
\multirow{2}{*}{Variable} & \multirow{2}{*}{Evaluation} & \multicolumn{6}{c}{Value}                     \\ \cline{3-8} 
                          &                             & 20    & 40    & 60    & 80    & 100   & 120   \\ \hline
\multirow{3}{*}{$N_r$}    & Recall@1                    & 0.871 & 0.874 & 0.869 & 0.869 & 0.873 & 0.871 \\ \cline{2-8}
                          & AUC                         & 0.996 & 0.996 & 0.997 & 0.996 & 0.995 & 0.994 \\ \cline{2-8}
                          & F1 max                      & 0.887 & 0.894 & 0.891 & 0.883 & 0.877 & 0.866 \\ \hline
\multirow{3}{*}{$N_e$}    & Recall@1                    & 0.872 & 0.873 & 0.871 & 0.872 & 0.866 & 0.871 \\ \cline{2-8}
                          & AUC                         & 0.996 & 0.996 & 0.996 & 0.996 & 0.997 & 0.996 \\  \cline{2-8}
                          & F1 max                      & 0.892 & 0.892 & 0.893 & 0.892 & 0.892 & 0.894 \\ \hline \bottomrule
\end{tabular}}
\label{table:abs_rsolid}
\vspace{-0.5cm}
\end{table}

%% ==========================================================================================================================================================================
% Additionally, we examine the success rate and correct rate of initial rotation based on $N_a$ in \textit{KITTI 08}.
% Success rate is defined as TPRE<6∘TP+FP\frac{TP_{RE<6^\circ}}{TP + FP} in recall@1 \cite{komorowski2021egonn, cattaneo2022lcdnet, xu2023ring++}, and correct rate is defined as TPRE<6∘TP\frac{TP_{RE<6^\circ}}{TP} in our letter.
% In other words, after estimating the initial rotation, it is the proportion of TP where the rotation error does not exceed 6∘^\circ.
% \begin{table}[h]
% \caption{Ablation Study For A-SOLiD}
% \renewcommand{\arraystretch}{1.2}
% \centering\resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|c|cccccccc}
% \toprule \hline
% \multirow{2}{*}{Variable} & \multirow{2}{*}{Evaluation} & \multicolumn{8}{c}{Value}                     \\ \cline{3-10} 
%                           &                             & 20   & 40     & 60     & 90     & 120    & 180    & 240    & 360   \\ \hline
% \multirow{2}{*}{NaN_a}    & Success Rate                & 0    & 0.020  & 0.040  & 0.072  & 0.076  & 0.078  & 0.078  & \textbf{0.078} \\ \cline{2-10}
%                           & Correct Rate                & 0    & 0.250  & 0.494  & 0.894  & 0.941  & 0.963  & 0.963  & \textbf{0.963} \\ \hline \bottomrule
% \end{tabular}}
% \end{table}

% \noindent Naturally, better results are expected as the descriptor becomes more dense.
% However, considering the increase in descriptor size, careful consideration is required to address the trade-off.

% \begin{figure}[h]
%     \centering
%     \def\width{0.98\columnwidth}
%     \includegraphics[clip, trim= 100 40 100 50, width=\width]{Figure/correct_rate/correct_rate.pdf}
%     \caption{Correct Rate.}
%     % \vspace{-0.5cm}
%     \label{fig:correct_rate}
% \end{figure}  
%% ==========================================================================================================================================================================

==> PaperWriting/introduction.tex <==
\section{Introduction}
\lettrine[lines=2] {L}\;\;ight detection and ranging (LiDAR) based \ac{PR} is a critical for the \ac{SLAM} problem highlighting the importance of environmental perception and map accuracy.
Unlike vision-based \ac{PR} methods \cite{cummins2008fab, galvez2012bags, arandjelovic2016netvlad, lee2021eventvlad, hsjang-2023-iros, kim2023robust} that have problems with illumination variations, visual changes, and time consumption in estimating 3D information, LiDAR \ac{PR} approaches \cite{rohling2015fast, he2016m2dp, cop2018delight, kim2018scan, wang2020lidar, cao2020season, vidanapathirana2022logg3d, ma2022overlaptransformer, lu2022one, lu2023deepring, xu2023ring++} have become more prominent because of the robustness of these constraints.
LiDAR \ac{PR} methods are integrated with LiDAR odometry estimation techniques \cite{zhang2014loam, shan2018lego, shan2020lio, xu2021fast, jung2023asynchronous} to form \ac{SLAM} \cite{kim2022sc}. 
These \ac{SLAM} approaches require the memory size of the onboard hardware to be considered.
This is because a mobile robot is equipped with a compact onboard computer that tends to have a reduced memory size and computing performance relative to desktop computers.
For instance, a compact device, such as a commercially available nano drone, functions on an embedded system with less than 1MB of RAM \cite{8046794}. 
Therefore, while employing sliding windows or filtering techniques, the fundamental issue of the size of stored descriptions remains unresolved \cite{9561638}.
In addition, lightweight descriptors are indispensable for efficient communication in a scenario where multiple mobile robots operate simultaneously.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[t]
% \caption{Main AUC Figure}
% \renewcommand{\arraystretch}{1.2}
% \centering\resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|c|ccccccc}
% \toprule \hline
% Score                     & FOV & Histogram & LoGG3D & M2DP  & SC    & OT    & Ring++ & Ours  \\ \hline
% \multirow{4}{*}{AUC/Size} & 60  & 1.040     & 0.420  & 0.562 & 0.058 & 0.837 & 0.003  & 2.208 \\
%                           & 120 & 1.036     & 0.423  & 0.576 & 0.039 & 0.805 & 0.003  & 2.219 \\
%                           & 180 & 1.041     & 0.422  & 0.565 & 0.058 & 0.787 & 0.003  & 2.221 \\
%                           & 360 & 1.059     & 0.451  & 0.593 & 0.098 & 0.852 & 0.003  & 2.223  \\ \hline
% \multirow{4}{*}{AUC/Time} & 60  & 3.171     & 33.69  & 16.47 & 5.615 & 140.2 & 0.458  & 58.58 \\
%                           & 120 & 1.634     & 28.42  & 9.041 & 8.168 & 104.8 & 0.461  & 45.46 \\
%                           & 180 & 1.128     & 24.91  & 6.415 & 5.477 & 84.17 & 0.461  & 37.80 \\
%                           & 360 & 0.588     & 16.08  & 3.356 & 3.111 & 45.67 & 0.442  & 20.84  \\ \hline \bottomrule
% \end{tabular}}
% \end{table}  

\begin{figure}[t]
	\centering
	\def\width{0.48\textwidth}%
    {%
		\includegraphics[clip, trim= 5 70 275 60, width=\width]{Figure/main_figure/main_figure.pdf}
	}
	\caption{At the top is our loop matching between the 1631st (red) and 192nd (yellow) frame in the \textit{KITTI 00} datasets clipped with a 60$^\circ$ Field of View (FOV).
             The loop matching exhibits slight differences in rotation.
             Our methodology (green) implies low points space, however, Scan Context (SC) (red) \cite{kim2018scan} signifies vacant information in the description.
             As the FOV narrows, it becomes more sensitive to subtle changes in small (purple) areas, and this directly correlates with success or failure.
             At the bottom is the weight-to-area under the curve (AUC) score graph.
             As the descriptor size increases, a more comprehensive description that effectively represents the scene is generated and the loop searching time is extended. 
             In essence, a trade-off comes into play, and the effectiveness of this graph signifies how well it can overcome this limitation.
             We compare our method with well-known methods in LiDAR \ac{PR} \cite{rohling2015fast, he2016m2dp, kim2018scan, vidanapathirana2022logg3d, ma2022overlaptransformer, xu2023ring++} where discussed in Section \uppercase\expandafter{\romannumeral2}-A.
             Our performance is about 2$\times$ $\sim$ 1000$\times$ superior to Histogram $\sim$ State Of The Art (SOTA)~Ring++.
             }
        \vspace{-0.5cm}
	\label{fig:main}
\end{figure}

% Traditional \ac{SLAM} approaches have primarily been designed for spinning \ac{LiDAR}. 
% However, spinning \ac{LiDAR} collects all points surrounding the sensor, resulting in extensive computation.
% Recently, these LPRs play an axiomatic role in stable autonomous driving \cite{shi2023lidar} to navigate the correct route. 
% For a LiDAR \ac{PR} to be universally applicable, it must exhibit robustness against various FOVs.
In various autonomous vehicles and robot platforms, systems commonly utilize LiDAR in limited FOV.
% Because the LiDAR's specific view has been employed recently, 
Moreover, when fusion is employed to enhance perception performance, it often encounters situations where the FOV is restricted, as illustrated in \figref{fig:limited_fov}, such as LiDAR object detection \cite{wang2018pointseg, wu2018squeezeseg, wu2019squeezesegv2, aksoy2020salsanet}, and LiDAR-camera fusion \ac{SLAM} \cite{shin2020dvl}. 
This fusion typically utilizes only the overlapping LiDAR views with camera information, negating the need to process all 360$^\circ$ data.
Thus, points disregarded by perception merely occupy computer memory without contributing to the analytical process, rendering their retention unnecessary.
% LiDAR object detection \cite{wang2018pointseg, wu2018squeezeseg, wu2019squeezesegv2, aksoy2020salsanet} demonstrates its capability to effectively segment dynamic objects and the ground in the front view, providing valuable assistance for driving.
% LiDAR-camera fusion \ac{SLAM} \cite{shin2020dvl} systems have emerged, enabling the creation of denser maps. 
% Also, the LiDAR dataset \cite{kim2020mulran} designed for LPR is configured with predominantly excluded rearward views.
% Likewise, they also have challenges arising from long-term mechanical issues such as twisted rotation axis or occlusion and unresolved high energy consumption.
% To address spinning LiDAR's mechanical components, offering affordability, durability, and suitability in environments with temperature changes or intense vibrations, solid-state \ac{LiDAR} has emerged. 
% To address spinning LiDAR's limitations, solid-state \ac{LiDAR} has emerged. 
Owing to these purposes, solid-state LiDAR has made remarkable progress and public datasets have been increasingly focusing on front views \cite{kim2020mulran, lee2023conpr, jung2023helipr}.
It excels in highly mobile robots, providing denser points even within a narrow FOV owing to its high update frequency and angular resolution, as evidenced by its applications in the delivery robot market \cite{9981281}.
Accordingly, to its development, mapping algorithms \cite{lin2020loam, liu2021balm} for solid-state LiDAR capabilities appear. 
However, due to solid-state LiDAR's narrow FOV, these approaches lose key features during movement along walls or abrupt FOV changes, resulting in a lower localization accuracy than that of 360$^\circ$ FOV LiDAR \cite{zhou2023comparative}.
Moreover, in the event of occlusion caused by LiDAR malfunctions, points may enter at random angles, directly affecting the localization accuracy.
Therefore, odometry may become compromised and increase uncertainty, and a pose correction step using LiDAR \ac{PR} is imperative to overcome these limitations.
Thus, in this letter, we propose a spatially organized and lightweight global descriptor called \textit{SOLiD} for LiDAR \ac{PR} to provide robustness against limited FOV and occlusions. 
The proposed method incorporates the following attributes:
\begin{itemize}
    \item Our descriptor is lightweight because of its rich spatial encapsulation. 
          As shown in \figref{fig:main}, its performance overwhelmingly excels in weight efficiency, making it well-suited for deployment on onboard computers with limited memory.
          Furthermore, our proposed approach can be applied via quick communication time in multi-robot scenarios.
    \item Despite employing brute-force search for comparison with other methodologies, our search speed is breakneck.
          In practical usage, we identify a significant improvement in the search speed by constructing a kd-tree.
    \item Our method can be applied not only to solid-state LiDAR but also to spinning LiDAR with limited FOV. Specifically, our methodology demonstrates robustness to occlusion.
    \item Owing to the nature of lightweight descriptors, there is a significant loss of information, which makes it challenging to estimate the initial rotation. 
          Despite this difficulty, we can estimate the initial rotation, which can contribute to the accuracy of \ac{SLAM}.
\end{itemize}

% Our remaining paper is structured as follows: Section\uppercase\expandafter{\romannumeral2} describes related works. 
% Section \uppercase\expandafter{\romannumeral3} introduces detailed information about our description and PR, particularly explaining how our description is spatially organized. 
% Section \uppercase\expandafter{\romannumeral4} compares our method with other approaches, dividing the comparison into intra-session, inter-session, and distributed-session in desktop and onboard computer. 
% Finally, Section \uppercase\expandafter{\romannumeral5} consists of the summary and conclusion including future works.



==> PaperWriting/limitation.tex <==
\section{Limitation}
In LiDAR PR research, most approaches determine correct/incorrect matching pairs based on the ground truth translation.
However, in limited FOV scenarios, when a robot navigates in the opposite direction to a revisited place, an overlapping region of the LiDAR views between the current place and the revisited place may not occur, or only the vertical plane in the direction of progress may overlap, even if the translation difference is a little apart.
Therefore, it decreases the performance of metrics such as Recall@1, which are calculated based on the number of ground truth matching pairs.
% In other words, even if the overlap of the LiDAR views between the current place and the revisited place is minimal or nonexistent, it still counts towards the number of ground truths.
% This decreases the Recall@1 performance of our method and that of any other methods.
% However, in limited FOV scenarios, if a robot navigates to a revisited place in the opposite direction, there won't be overlapping regions at the same location. 
% As with any other method, the proposed method also faces this issue. 
% Our descriptor can recognize the revisited places and estimate the initial heading in the same direction with slight overlapping areas, as shown in \figref{fig:main}.
% However, our method cannot find reverse loops with no overlapping regions.
Thus, in LiDAR PR research utilizing narrow FOV, a new metric for selecting ground truths should be proposed that leverages rotation and translation similar to visual PR \cite{gao2022airloop, schubert2023visual}.

==> PaperWriting/problem.tex <==
\section{Problem Formulation}
In this section, we analyze the limitations of the traditional LiDAR \ac{PR}. 
Noteworthy is the difficulty of dealing with various situations owing to the challenging design of accommodating diverse FOVs.
Furthermore, traditional methods tend to prioritize performance, often overlooking loop searching time.
In this letter, we propose a method that enables spinning LiDAR and solid-state LiDAR to concentrate on limited FOV, reduce the number of points required, and enable more efficient computations.
While simultaneously achieving high performance and fast searching times, we generate sophisticated encapsulation using a radial-wise \textit{R-SOLiD} and azimuthal-wise \textit{A-SOLiD}.
Our descriptor follows the pipeline as represented in \figref{fig:pipeline}, which ensures a more efficient pre-processing stage.

\subsection{Limitation in Limited FOV}
When the FOV is restricted, the reduced number of bins in the constructed Histogram makes it challenging to effectively describe the current scene.
Moreover, due to the constrained range of principal components, M2DP exhibits performance limitations, and the reduction in the number of local features leads to a decrease in the performance of LoGG3D. 
Additionally, when the orientation exceeds 180$^\circ$, 50$\%$ of the range image becomes vacant space, causing a loss of functionality in OT.
Furthermore, 8 bins in DeLight transform into empty space.
Similarly, SC becomes disabled as the description itself contains more than 50$\%$ blank space.
Ring and Ring++ benefit from the construction of rays from the RT, providing a relatively unrestricted capability in dealing with vacant spaces.
However, beneath this lies an inherent limitation for real-time performance, as the focus has been primarily on optimizing for overall performance.

\subsection{Trade-off according to descriptor size}
The LiDAR \ac{PR} can be broadly categorized into three stages: place description, which explains the current location; loop detection, which identifies revisited places based on the description; and pose estimation, which determines the relative pose between the current location and revisited places.
In LiDAR \ac{PR}, as the description becomes more captured, performance can only be expected to improve.
However, in terms of complexity, portraying a scene lies in the hidden inefficiency of time-consuming loop searching.
Similarly, as the scene becomes more condensed, the performance decreases, but this allows for rapid search times.
Therefore, a spatially organized description is necessary to encapsulate the current place effectively.
